SHAP Meets Tensor Networks: Provably Tractable Explanations with Parallelism

Although Shapley additive explanations (SHAP) can be computed in polynomial time for simple models like decision trees, they unfortunately become NP-hard to compute for more expressive black-box models like neural networks - where generating explanations is often most critical. In this work, we analyze the problem of computing SHAP explanations for *Tensor Networks (TNs)*, a broader and more expressive class of models than those for which current exact SHAP algorithms are known to hold, and which is widely used for neural network abstraction and compression. First, we introduce a general framework for computing provably exact SHAP explanations for general TNs with arbitrary structures. Interestingly, we show that, when TNs are restricted to a *Tensor Train (TT)* structure, SHAP computation can be performed in *poly-logarithmic* time using *parallel* computation. Thanks to the expressiveness power of TTs, this complexity result can be generalized to many other popular ML models such as decision trees, tree ensembles, linear models, and linear RNNs, therefore tightening previously reported complexity results for these families of models. Finally, by leveraging reductions of binarized neural networks to Tensor Network representations, we demonstrate that SHAP computation can become *efficiently tractable* when the network's *width* is fixed, while it remains computationally hard even with constant *depth*. This highlights an important insight: for this class of models, width - rather than depth - emerges as the primary computational bottleneck in SHAP computation.

==> assets/DT2TT.tex <==
\begin{figure}[htbp]
\centering

% --- Row 1: Decision Tree + FSM Lattice ---
\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{tikzpicture}[scale=0.9, every node/.style={font=\small}]
  % Decision tree nodes
  \node[circle,draw] (x1) at (0,0) {$x_1$};
  \node[circle,draw] (x2a) at (-2,-1.5) {$x_2$};
  \node[circle,draw] (x2b) at (2,-1.5) {$x_2$};

  % Leaves as rounded rectangles
  \node[draw,rounded corners,fill=yellow!40,minimum width=0.6cm,minimum height=0.4cm] (y00) at (-3,-3) {$0$};
  \node[draw,rounded corners,fill=green!40,minimum width=0.6cm,minimum height=0.4cm] (y01) at (-1,-3) {$1$};
  \node[draw,rounded corners,fill=yellow!40,minimum width=0.6cm,minimum height=0.4cm] (y10) at (1,-3) {$0$};
  \node[draw,rounded corners,fill=green!40,minimum width=0.6cm,minimum height=0.4cm] (y11) at (3,-3) {$1$};

  % Edges
  \draw[-{Stealth}] (x1) -- (x2a) node[midway,above left] {$0$};
  \draw[-{Stealth}] (x1) -- (x2b) node[midway,above right] {$1$};

  \draw[-{Stealth}] (x2a) -- (y00) node[midway,above left] {$0$};
  \draw[-{Stealth}] (x2a) -- (y01) node[midway,above right] {$1$};

  \draw[-{Stealth}] (x2b) -- (y10) node[midway,above left] {$0$};
  \draw[-{Stealth}] (x2b) -- (y11) node[midway,above right] {$1$};
\end{tikzpicture}
\subcaption*{(a) Decision tree}
\end{subfigure}

\hfill
\begin{subfigure}[b]{0.7\textwidth}
\centering
\begin{tikzpicture}[scale=0.9, every node/.style={font=\small}] 
  % Four FSMs arranged vertically
  \foreach \i in {0,1}{
    \pgfmathsetmacro{\yshift}{-(\i)*1.4}
    \pgfmathtruncatemacro{\j}{mod(\i + 1, 2)}
    % States (horizontal)
    \node[circle,draw,minimum size=20pt, initial] (s0\i) at (0,\yshift) {};
    \node[circle,draw,minimum size=20pt] (s1\i) at (2.0,\yshift) {};
    \node[circle,draw,minimum size=20pt, fill=green!30, accepting] (s2\i) at (4.0,\yshift) {};
    % Transitions
    \draw[-{Stealth}] (s0\i) -- (s1\i) node[midway,above] {$x_1 =$\i};
    \draw[-{Stealth}] (s1\i) -- (s2\i) node[midway,above] {$x_2 =1$};
  }
\end{tikzpicture}

\subcaption*{(b) Lattice of finite-state machines}
\end{subfigure}

\vspace{1em}

% --- Row 2: Tensor Train ---
\begin{subfigure}[b]{0.4\textwidth}
\centering\begin{tikzpicture}[every node/.style={draw, minimum size=0.7cm, font=\small}]
  % Tensor train nodes
  \node[circle] (G1) at (0,0) {$G^{(1)}$};
  \node[circle] (G2) at (2,0) {$G^{(2)}$};

  % Edges with labels (nodes without the 'draw' option)
  \draw[-] (G1) -- ++(0,-0.8) node[below, draw=none] {$x_1$};
  \draw[-] (G2) -- ++(0.8,0) node[right, draw=none] {$y$};
  \draw[-] (G1) -- (G2);
  \draw[-] (G2) -- ++(0,-0.8) node[below, draw=none] {$x_2$};
\end{tikzpicture}
\subcaption*{(c) Tensor Train representation}
\end{subfigure}

\caption{Progressive mapping from (a) a simple decision tree, to (b) its equivalent lattice of finite-state machines, and finally to (c) the corresponding Tensor Train representation. The TT cores are \(G^{(1)} \in \mathbb{R}^{1 \times 2 \times r_1}\) and \(G^{(2)} \in \mathbb{R}^{r_1 \times 2 \times 1}\).}
\label{fig:tree_fsm_tt}
\end{figure}


==> assets/tensorshap.tex <==
\begin{tikzpicture}[
    node distance=0.8cm and 1cm,
    every node/.style={inner sep=1pt}
  ]

  % Top: T^M
  \node[rect] (TM) at (0,3) {\(\mathcal{T}^M\)};

  % Middle row: M1, M2, M3
  \node[circ, below=of TM.south, xshift=-3cm] (M1) {\(M_1\)};
  \node[circ, below=of TM.south]                  (M2) {\(M_2\)};
  \node[circ, below=of TM.south, xshift= 3cm] (M3) {\(M_3\)};

  % Lower row: Tensor train G1..G4
  \node[circ, below=of M2.south, xshift=-4cm] (G1) {\(G_1\)};
  \node[circ, right=of G1]                  (G2) {\(G_2\)};
  \node[circ, right=of G2]                  (G3) {\(G_3\)};
  \node[circ, right=of G3]                  (G4) {\(G_4\)};

  % Bottom: T^P placed just below G3
  \node[rect, below=1cm of G3.south] (TP) {\(\mathcal{T}^P\)};

  % TM → Mi
  \draw[leg] (TM.south west) -- (M1.north);
  \draw[leg] (TM.south)      -- (M2.north);
  \draw[leg] (TM.south east) -- (M3.north);

  % Free legs x_i
  \draw[freeleg] (M1.west) -- ++(-0.6,0) node[left]{\(x_1\)};
  \draw[freeleg] (M2.west) -- ++(-0.6,0) node[left]{\(x_2\)};
  \draw[freeleg] (M3.west) -- ++(-0.6,0) node[left]{\(x_3\)};

  % Mi → G_{i+1}
  \draw[leg] (M1.south) -- (G2.north);
  \draw[leg] (M2.south) -- (G3.north);
  \draw[leg] (M3.south) -- (G4.north);

  % Connect the Tensor Train chain
  \draw[leg] (G1) -- (G2);
  \draw[leg] (G2) -- (G3);
  \draw[leg] (G3) -- (G4);

  % TP → G2,G3,G4
  \draw[leg] (TP.north west) -- (G2.south east);
  \draw[leg] (TP.north)      -- (G3.south);
  \draw[leg] (TP.north east) -- (G4.south west);

  % Free leg Y on TP
  \draw[freeleg] (TP.south) -- ++(0,-0.6) node[below]{\(Y\)};

\end{tikzpicture}
